NEREL-BIO: A Dataset of Biomedical Abstracts Annotated with Nested Named Entities

This paper describes NEREL-BIO -- an annotation scheme and corpus of PubMed abstracts in Russian and smaller number of abstracts in English. NEREL-BIO extends the general domain dataset NEREL by introducing domain-specific entity types. NEREL-BIO annotation scheme covers both general and biomedical domains making it suitable for domain transfer experiments. NEREL-BIO provides annotation for nested named entities as an extension of the scheme employed for NEREL. Nested named entities may cross entity boundaries to connect to shorter entities nested within longer entities, making them harder to detect. NEREL-BIO contains annotations for 700+ Russian and 100+ English abstracts. All English PubMed annotations have corresponding Russian counterparts. Thus, NEREL-BIO comprises the following specific features: annotation of nested named entities, it can be used as a benchmark for cross-domain (NEREL -> NEREL-BIO) and cross-language (English -> Russian) transfer. We experiment with both transformer-based sequence models and machine reading comprehension (MRC) models and report their results. The dataset is freely available at https://github.com/nerel-ds/NEREL-BIO.

==> old_do_not_use.tex <==
\section{Introduction}
There has been a growth of interest in automatic methods of information extraction from biomedical texts in multiple languages including not just English but Spanish, French, Russian etc. \cite{todo-Elena}. Historically datasets in the biomedical domains have been created for English \cite{todo-Elena} while there are a smaller number of annotated biomedical datasets in other languages \cite{todo-Elena}.
%During last years there is a great interest to automatic methods of information extraction from biomedical texts including scientific abstracts, clinical records, and social network posts \citep{karimi2015cadec,tutubalina2021russian,sboev2022analysis}. Of all these sources, clinical texts are the least accessible due to the fact that they involve personal data. 

In this paper, we describe NEREL-BIO dataset, 
%the first 
a Russian dataset of scientific abstracts annotated with biomedical entities. NEREL-BIO extends existing annotation scheme developed in NEREL \cite{NEREL} with additional xx of entity types. These cover diseases and related medical procedures such as treatment or laboratory tests. 
%The chosen topic of the dataset allows providing additional annotated data for processing clinical documents in Russian.\pb{remove or explain, why}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.4\textwidth, height=25mm] 
    {bio_example.eps}
    \caption{Example of nested named entities in NEREL-BIO. Internal entities ``bronchus'', ``bronchus resection'', ``resection'' are available in UMLS. Longer entities ``isolated bronchus resection'' and ``central cancer'' are important for establishing appropriate relations. %\pb{move Figure to page 2?}
    }
    \label{fig:example}
\end{figure} 


%\pb{Too short for a separate section? Move to intro?}
%\pb{Need to add some examples and discussion}

Our work has four goals:
\begin{itemize} 
\item\ create a Russian corpus of scientific biomedical abstracts;
%Such abstracts are maximally closer in content to clinical notes, which are usually  poorly accessible; 
%\pb{Reviewer might say why then not use clinical notes datasets}
\item\ annotate nested named entities and relations between nested entities;
%which gives possibility to study various algorithms for information extraction over nested named entities;
\item\ develop a broader unified annotation scheme covering both the general and the  biomedical domains; 
\item\ provide annotation for a (smaller collection) parallel English abstracts using the same guidelines to study cross-lingual approaches.
\end{itemize}

NEREL-BIO extends the annotation scheme of the general-domain Russian dataset NEREL \citep{NEREL}. Both NEREL and NEREL-BIO are annotated with nested named entities, relations between entities, and  Wikidata links. This paper covers only named entities. Biomedical texts contain numerous nested mentions of entities such as anatomical parts within each other, diseases containing body parts or chemicals, procedures containing names of  diseases or devices, etc. For example, in \textit{colon cancer}, a body part (\textit{colon}) is contained in a disease name. Annotation on nested entities provides a structured mechanism for annotating and extracting relations, as well for entity linking to knowledge bases such as UMLS \citep{bodenreider2004unified}.

Fig~\ref{fig:example} presents an example of nested named entities in NEREL-BIO. It discusses isolated bronchus resection for central cancer, provides results of surgical treatment in these specific conditions. Entities ``bronchus'', ``bronchus resection'', ``resection'' are included in UMLS, while ``isolated bronchus resection'' and ``central cancer'' are not.  Nested entity annotations create a basis for  establishing relations between correct (longer) entities, as well as  linking internal entities to equivalent UMLS concepts. 


NEREL-BIO contains entities from the general domain to study domain transfer techniques. When many new entities appear in a specific domain, entity types from the general domain are also mentioned but their contexts were modified, in some cases annotation rules could change, some entity types could be renamed, while some general types becomes less frequent. With this aim, we start from 29 entity types of the NEREL corpus and add specialized biomedical entity types. %5When annotating NEREL-Bio, annotators have the choice of choosing entity types from NEREL together with additional NEREL-BIO specific biomedical entity types. This sharing of entity types enables transfer from the general domain. 

Additionally, NEREL-BIO corpus contains 100+ English documents annotated with the same annotation scheme which can be useful for studying cross-lingual transfer approaches.
%During the annotation we discovered that some entity types require renaming since they have different meaning in the biomedical domain. Other entities can be redefined in the domain with changing annotation rules, some general entities can be rare or absent in a domain-specific corpus. \pb{repetition? see previous paragraph}


 %NEREL is the first dataset annotated simultaneously with nested entities, relations between those entities and knowledge base links.  Such annotations pose challenges to current state-of-the-art relation extraction models that lack support for relations between nested and overlapping entities.  NEREL relations may lie inside a sentence or span across sentence boundaries. 
%Entity linking annotations leverage nested named entities, and each nested named entity can be linked to a separate Wikidata entity.  
%NEREL provides a novel testbed for sentence- and document-level relation extraction methods.

%At the time of writing, NEREL  is  the largest Russian dataset  annotated with entities and relations when compared to the existing Russian datasets. NEREL features the largest number of entity and relation types -- currently 29 and 49, respectively.  Currently, the dataset contains 56K named entities and 39K relations annotated in 900+ person-oriented news articles. 

\section{Related work}
Our work relates to three directions of biomedical entity annotation: disease-related annotation of biomedical abstracts, annotation of clinical records, and annotation of biomedical texts with UMLS concepts.
The most famous corpus for biomedical named entity recognition in English is GENIA~\citep{kim2003genia} that consists of 2,000 MEDLINE abstracts with more than
400,000 words and almost 100,000 annotations for
biological terms. The annotated abstracts are mainly devoted to biological reactions concerning transcription factors in human blood cells. 47 entity types organized in a taxonomy were annotated. The top three concepts include:   biological source, biological
substance and other concepts. The annotation includes nested and fragmented (non-continuous) entities. 

\cite{leaman2009enabling} developed the Arizona Disease Corpus (AZDC) that contains MEDLINE abstracts annotated with  disease mentions.  \cite{gurulingappa2010empirical} created a corpus of 400 annotated MEDLINE abstracts for human diseases and adverse effects. \cite{van2012eu} released a 
% publicly available 
corpus of 300 abstracts, where instances of drugs, disorders, genes, and relationships among the identified entities are annotated. 

Many studies are devoted to annotation and text mining of clinical texts (patient records) \citep{roberts2009building}. \cite{patel2018annotation} created a clinical entity recognition (CER) corpus of 5,160
clinical documents from 40 different clinical specialities using 11 entity types such as diseases, procedures, medications, medical devices, etc.; relations of five types were established between entities.

Some works annotate biomedical abstracts with UMLS concepts \citep{mohan2018medmentions,neveol2014quaero}. In such work named entity annotations are based on the upper-level concepts (superconcepts) of the UMLS ontology \citep{bodenreider2004unified,mccray2001aggregating}. \cite{mohan2018medmentions} describe MedMentions corpus, which is annotated with 21 UMLS superconcepts, including 
% traditional for biomedical texts 
annotation of disorders, anatomical structures, chemicals, and also some general concepts such as organizations, population groups, etc. \cite{neveol2014quaero} in their corpus Quaero exploit 10 UMLS superconcepts \cite{mccray2001aggregating} combining biomedical entity types and general types such as geographic areas. 

There exist a small number of  Russian corpora with annotations of biomedical texts for information extraction. \cite{shelmanov2015information} created a corpus of clinical notes \pb{records?} in the Russian language. The tasks of the work include: drug identification and disease
template filling, which are related to entity recognition and relation extraction.  The
disease template filling consists of recognition of disease mentions in text, mapping
them onto concepts of a thesaurus, and discovering their attributes.  The corpus  contains currently more than 112 fully annotated texts with almost
45,000 tokens. There are more than 7,600 annotated entities (seven entity types),  more than 4,000
annotated attributes (four attribute types) and relations.

Several studies are devoted to extracting of adverse drug reactions from Russian texts. \cite{alimova2017machine} created a Russian corpus of user reviews from the website Otzovik.com with four types of sentence annotations: indication, beneficial effect, adverse drug reactions, and `other'.
\cite{tutubalina2021russian} presented a corpus of consumer reviews about drugs. Each review is  annotated with six types of named entities: drug name, class and form, adverse drug reactions, drug indications and symptoms of a disease, and ”finding” (a miscellaneous type). The dataset with 4,566 entities. \cite{sboev2022analysis} created a Russian corpus of 2,800 user reviews about drug reactions. 
% The corpus includes 2800 users' reviews. 
The annotation includes medications with ten  attributes (such as dosage or manufacturer), diseases for that medications are prescribed and their six attributes \pb{??}, adverse drug reactions. The annotation comprises discontinuous and overlapping entities. Altogether, 52,186 entities were annotated.

In 2022, \cite{blinov2022rumedbench} announced RuMedBench, a Russian Medical Language Understanding Benchmark.\footnote{\url{https://github.com/pavel-blinov/RuMedBench}} The RuMedBench contains five tasks based on four medical text types including: (i)~RuMedTop3 for diagnosis prediction, (ii)~RuMedSymptomRec for symptoms recommendation, (iii)~RuMedDaNet for medical Question Answering (QA), (iv)~RuMedNLI, the translated version of
the medical Natural Language Inference (NLI) task, and (v)~previously created RuMedNER for  named entity recognition in drug-related user reviews \citep{tutubalina2021russian}. 

In this work, we describe a corpus NEREL-BIO of medical abstracts in Russian, which discuss various diseases and their treatment. The corpus contains discussion of a wide variety of  diseases and their treatments. This means that corpus content is maximally close to the content of clinical notes and the corpus can be used as an additional dataset for training models for clinical notes analysis. \pb{move to intro?}

